A Competitive Posted-Price Mechanism for Online Budget-Feasible Auctions

We consider online procurement auctions, where the agents arrive sequentially, in random order, and have private costs for their services. The buyer aims to maximize a monotone submodular value function for the subset of agents whose services are procured, subject to a budget constraint on their payments. We consider a posted-price setting where upon each agent's arrival, the buyer decides on a payment offered to them. The agent accepts or rejects the offer, depending on whether the payment exceeds their cost, without revealing any other information about their private costs whatsoever. We present a randomized online posted-price mechanism with constant competitive ratio, thus resolving the main open question of (Badanidiyuru, Kleinberg and Singer, EC 2012). Posted-price mechanisms for online procurement typically operate by learning an estimation of the optimal value, denoted as OPT, and using it to determine the payments offered to the agents. The main challenge is to learn OPT within a constant factor from the agents' accept / reject responses to the payments offered. Our approach is based on an online test of whether our estimation is too low compared against OPT and a carefully designed adaptive search that gradually refines our estimation.

==> Predictions.tex <==
    \section{Mechanism with Predictions}
In the following we will suppose that apart from our input $(\mathcal{N},B)$ we are also given a prediction $\hat{t}$, a recommended value for the threshold parameter. We will present how to achieve a smooth transition between the $O(1)$ consistency and $O(\log\log n \log \log\log n)$ robustness, depending on the error of the given prediction. 

We will call this mechanism $ProcurementPrediction$. The main idea behind it is to split the mechanism at two phases. Each phase will consist of $\ell$ rounds constructed exactly as in the \ref{alg:Init}.
\subsection{Phase A}
During phase A we will begin by applying threshold $\hat{t}$ at the first round. If the round is successful, we will double the threshold, else we halve it. We can view this procedure as a random walk where the state space is a discretized array of threshold values. This random walk is heavily drifted towards thresholds greater than $\frac{f(OPT)}{7}$. Phase B will be exactly the same as \ref{alg:FINAL}.

We present the complete $ProcurementPrediction$ mechanism, formally written in pseudocode:

\begin{algorithm}[H]
\caption{PREDICTION-MECHANISM}\label{alg:PRED}
\begin{algorithmic}[1]
\STATE \textbf{Input}: Set of agents $\mathcal{N}$, budget $B$, at each timestep $i \in [n]$ an agent $b(i)$ in random order.
\STATE \textbf{Initialize:} Timestep $i=0$, solution $S =\emptyset$
\STATE
    \STATE $i=0$
    \FOR{$j \in [2\ell]$}
    \STATE Draw $n_j$ from $Bi(n-i,a)$.
    \STATE $i \gets i+ n_j$.
    \ENDFOR
\STATE
    \FOR{$j\in [\ell]$}
    \IF{$TestThreshold([b(i),\dots, b(i+n_j-1)],\hat{t}) > 0$ }{
        \STATE$\hat{t} \gets 2\cdot \hat{t}$
    }
    \ELSE{
        \STATE $\hat{t} \gets \hat{t} / 2$
    }
    \ENDIF
    \ENDFOR
    \STATE Construct $d$ using the agent with the highest utility observed till now, then conduct binary search like before.
\end{algorithmic}
\end{algorithm}

 To understand why our mechanism works we will investigate the overall value achieved from the following random walk:
 \begin{definition}
     $\mathcal{M}_1$ is a Markov Chain with states $\{\dots,-1,0,1,\dots\}$, where being in state $i$ means that we use threshold $2^{-i}\cdot \hat{t}$, and 
 the transition probabilities at a round $j$ are the following:
 \begin{equation}
 \begin{split}
          \Prob{S_{j+1} = i-1| S_{j} = i} &= \Prob{\text{round } j \text{ succeeds while using threshold } 2^{-i}\cdot \hat{t}}\\
     \Prob{S_{j+1} = i+1| S_{j} = i}& = \Prob{\text{round } j \text{ fails while using threshold } 2^{-i}\cdot \hat{t}}
 \end{split}
 \end{equation}
 \end{definition}
This random walk models the exact behaviour of our mechanism. To simplify the analysis of the random walk we investigate the competitive ratio of our mechanism under the following assumption:
\begin{assumption}\label{ass1}
All thresholds greater than $\frac{f(OPT)}{7}$ fail in all rounds.    
\end{assumption}
 It is evident that this way we underestimate the actual competitive ratio of our mechanism. Another problem are the time-varying and unknown transition probabilities that make a complete analysis hard. To tackle this, we study Markov Chains with "worse", but constant, success probabilities than $\mathcal{M}_1$. Proving the desired results in these simplified Markov Chains we manage to transfer them to $\mathcal{M}_1$ by properly coupling them. A complete analysis is available at the appendix.

Let $i^{*}$ be the smallest integer such that $2^{-i^{*}}\cdot \hat{t} \le \frac{f(OPT)}{7}$. To simplify even further our analysis, we take into account the utility achieved only from state $i^{*}$. 

 Our main lemmas are the following:
\begin{lemma}\label{lemSteps}
    With probability at least $0.5$ Random walk $\mathcal{M}_1$ reaches state $i^{*}$ after $\frac{|i^{*}|}{0.8}$ rounds.
\end{lemma}

The lemma above signifies the drift towards $\frac{f(OPT)}{7}$. The following lemma suggests that once our mechanism has reached $i^{*}$ it will make many visits to it again. 

\begin{lemma}\label{lemReturn}
    If random walk $\mathcal{M}_1$ is in state $i^{*}$ and there are $r$ rounds left, then with probability at least $0.5$ it will return at least $\left\lfloor r\cdot 0.49\right\rfloor$ times to it again.
\end{lemma}
We are now ready to prove our main theorem of mechanism \ref{alg:PRED}.

\begin{theorem}
    Mechanism \ref{alg:PRED} is $O(1)$ consistent and $O(\log\log n\log\log\log n)$ robust.
\end{theorem}
\begin{proof}
    We begin by considering the following cases:
    \begin{enumerate}
        \item Prediction is inaccurate, namely $\max\left\{ \log \left(\frac{\hat{t}}{f(OPT)}\right),\log\left (\frac{f(OPT)}{\hat{t}}\right)\right\} > \log\log n \cdot \log\log\log n $. In this case, we ignore phase A, and we have guaranteed $O(\log\log n \log\log\log n)$  competitive ratio by the second phase where we conduct binary search.
        \item Prediction is accurate, namely $\max\left\{ \log \left(\frac{\hat{t}}{f(OPT)}\right),\log\left (\frac{f(OPT)}{\hat{t}}\right)\right\} > \log\log n \cdot \log\log\log n $. We will showcase how the competitive ratio is improved in this case. Firstly, we should note that in this case the following holds $|i^{*}|<3\log\log n \log\log\log n$. We consider two cases again:
        \begin{enumerate}
            \item $i^* > 0$:
             In this case, the worst scenario is for all rounds in  states  less than $i^*$ to fail, as in any other case we will have accumulated greater utility. Thus, we can suppose that after exactly $i^*$ rounds we have reached  state $i^*$., and according to lemma \ref{lemReturn} it will return another $\left\lfloor (\ell - i^*)\cdot 0.49\right\rfloor$ times. Combining this with lemma \ref{lemmaJustify} we get the following bound for the utility of our mechanism:
            \begin{equation}
                \begin{split}
                    \E{}{Pred(\mathcal{N},\hat{t},B)} \ge \underbrace{0.5 \cdot (1+\left\lfloor (\ell - i^*)\cdot 0.49\right\rfloor )}_{\text{expected number of visits to } i^*}\cdot \underbrace{0.9 \cdot C_2 \cdot a \cdot \frac{f(OPT)}{14}}_{\text{expected utility from a visit to }i^*}
                \end{split}
            \end{equation}
            \item $i^* \le 0$:
            In this case we use lemma \ref{lemSteps} to argue that with probability at least $0.5$ our mechanism will reach state $i^*$ after at most $\frac{|i^{*}|}{0.8}$ rounds. Now applying lemma \ref{lemReturn}, we get that with probability at least $0.5$ it will return to $i^*$ at least $\left\lfloor (\ell - \frac{|i^{*}|}{0.8})\cdot 0.49\right\rfloor$ times. Finally, applying lemma \ref{lemmaJustify} we get the following bound:
            \begin{equation}
                \begin{split}
                    \E{}{Pred(\mathcal{N},\hat{t},B)} \ge \underbrace{0.5\cdot 0.5 \cdot \left[1+\left\lfloor \left(\ell - \frac{|i^{*}|}{0.8}\right)\cdot 0.49\right\rfloor \right]}_{\text{expected number of visits to } i^*}\cdot \underbrace{0.9 \cdot C_2 \cdot a \cdot \frac{f(OPT)}{14}}_{\text{expected utility from a visit to }i^*}
                \end{split}
            \end{equation}
        \end{enumerate}
    \end{enumerate}
\end{proof}
